Monte Cimone: Paving the Road for the First Generation of RISC-V High-Performance Computers

The new open and royalty-free RISC-V ISA is attracting interest across the whole computing continuum, from microcontrollers to supercomputers. High-performance RISC-V processors and accelerators have been announced, but RISC-V-based HPC systems will need a holistic co-design effort, spanning memory, storage hierarchy interconnects and full software stack. In this paper, we describe Monte Cimone, a fully-operational multi-blade computer prototype and hardware-software test-bed based on U740, a double-precision capable multi-core, 64-bit RISC-V SoC. Monte Cimone does not aim to achieve strong floating-point performance, but it was built with the purpose of "priming the pipe" and exploring the challenges of integrating a multi-node RISC-V cluster capable of providing an HPC production stack including interconnect, storage and power monitoring infrastructure on RISC-V hardware. We present the results of our hardware/software integration effort, which demonstrate a remarkable level of software and hardware readiness and maturity - showing that the first generation of RISC-V HPC machines may not be so far in the future.

==> sections/07-Conclusions.tex <==
\section{Conclusions}  \label{sec:conclusion}

% \section{Code access}
%  Code for a classifier, implemented in this work is accessible at: \url{https://github.com/MolanM/TrueExplain}

% \section{Acknowledgements}

% This research was partly supported by the H2020-JTI-EuroHPC-2019-1 Regale project (g.a. 956560).


==> sections/figures/HPLandSTREAM.tex <==
\begin{figure}
\begin{minipage}{.4\linewidth}

    \centering
    \caption{STREAM, 4 threads} 
    \label{table:stream}
    \vspace{0.1in}
    
    \begin{tabular}{@{}lrr@{}} 
    \toprule
        \multirow{2}{*}{Test} &
        \multicolumn{1}{c}{\texttt{STREAM.DDR}} &
        \multicolumn{1}{c}{\texttt{STREAM.L2}} \\

        \cmidrule(lr){2-3}
        &
        1945.5 MiB [MB/s] &  % STREAM.DDR
        1.1 MiB [MB/s] \\  % STREAM.L2
        
        \midrule
        
        \texttt{copy}  & $1206 \pm 3.26$ & $7079 \pm 2.11$ \\
        \texttt{scale} & $1025 \pm 4.94$ & $3558 \pm 3.72$ \\
        \texttt{add}   & $1124 \pm 4.93$ & $4380 \pm 3.72$ \\
        \texttt{triad} & $1122 \pm 5.63$ & $4365 \pm 3.56$ \\

        \bottomrule
    \end{tabular}
    
\end{minipage}

\begin{minipage}{.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/hpl_strong_speedup.pdf}
        \caption{Relative speedup during HPL strong scaling tests on Monte Cimone. Average attained throughput values are shown in labels. Standard deviations are calculated on a population of 10 data points.}
        \label{fig:hpl_strong_scaling}
    \end{minipage}
\end{figure}




==> sections/figures/figura.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.5in]{img/exploration.pdf}
    \caption{Caption}
    \label{fig:exploration}
\end{figure*}


==> sections/tables/power_line_specs.tex <==
\begin{table}
    \centering
    \caption{Power line specifications}
    \label{table:power_line_specs}
    \vspace{0.1in}
    
    \begin{tabular}{@{}llrr@{}} 
        \toprule
        \multirow{2}{*}{Line} & 
        \multirow{2}{*}{Endpoint} & 
        \multicolumn{1}{c}{Shunt} & 
        \multicolumn{1}{c@{}}{Voltage} \\
        
        & 
        &
        \multicolumn{1}{c}{[m$\Omega$]} & 
        \multicolumn{1}{c@{}}{[V]} \\
        
        \midrule
        \texttt{core}     & FU740 core  & 1   & 0.919 \\
        \texttt{ddr\_soc} & FU740 core  & 1   & 1.197 \\
        \texttt{io}       & FU740 core  & 200 & 1.793 \\
        \texttt{pll}      & FU740 core  & 200 & 1.794 \\
        \texttt{pcievp}   & FU740 core  & 1   & 0.923 \\
        \texttt{pcievph}  & FU740 core  & 1   & 1.793 \\
        \texttt{ddr\_mem} & DDR4 memory & 1   & 1.197 \\
        \texttt{ddr\_pll} & FU740 core  & 200 & 0.920 \\
        \texttt{ddr\_vpp} & DDR4 memory & 1   & 2.443 \\
        \bottomrule
    \end{tabular}
\end{table}

